The volume-filtering immersed boundary method

We present a novel framework to deal with static and moving immersed boundaries (IB). In this strategy, called Volume-Filtering Immersed Boundary (VFIB) method, transport equations are derived by filtering the Navier-Stokes equations and accounting for stresses at the solid-fluid interface. The result is that boundary conditions that normally apply on the interface are transformed into bodyforces that apply on the right-hand side of the filtered transport equations. The filter width acts as a parameter that controls the level of resolution. The IB is considered well-resolved if the filter width is much smaller than the characteristic corrugation scale of the interface. There are several innovations in this IB method. First, it sheds light on the role of the internal flow which arises when the transport equations are solved inside the IB. We show that, it is essential to separate stresses due to the external and internal fluids in order to get accurate forces and provide a method to do so. Second, we show that volumes associated with Lagrangian forcing points on the boundary depend on the local topology of the surface. We provide a method to compute these volumes using a triangle tessellation of the interface and the surface density function. Third, we provide an efficient procedure to compute the solid volume fraction, thus, enabling tagging interior/exterior cells. This volume fraction is also involved in the procedure to separate stresses due to the external fluid from the total stresses. Fourth, we show a path forward to extend the VFIB method to Large Eddy Simulations involving IBs. Lastly, we apply the VFIB in several numerical tests involving two- and three- dimensional static and moving IBs. We show greatly improved results compared to prior IB methods. Further, we test several filter kernels and show that, for well-resolved IBs, the choice of the kernel plays little role.

==> sections/naca_0008.tex <==
\subsection{\textcolor{blue}{Flow past an airfoil}}
\label{sssec:airfoil}

{\color{revision}
In this section we show the ability of the VFIB method to solve for non-spherical shapes as well. Similar to test case presented by \citet{mittalVersatileSharpInterface2008}, we take the case of a NACA 0008 airfoil and simulate it at an angle of attack, $\alpha = 4^\circ$. A chord based Reynolds number of $\mathrm{Re}_c = 6000$ is chosen. Similar to \citet{mittalVersatileSharpInterface2008}, we take a domain size of $12c$ in the streamwise direction and $9c$ in the wall-normal direction where $c$ is the chord length of the airfoil. We match the resolution of the case to \citet{mittalVersatileSharpInterface2008} domain an have a resolution of 12 points across the leading edge of the boundary layer. The timestep of the simulation is chosen such that the maximum CFL number is 0.25. Figure \ref{fig:naca_cdcl} shows the coefficient of lift and drag as a function of non-dimensional time $t U_\infty /c$.}

\begin{figure}\centering
	\begin{subfigure}{0.45\linewidth}
    \includegraphics[width=\linewidth]{data/PDF/naca_cd.pdf}
    \caption{\label{fig:cd_naca}}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
	\includegraphics[width=\linewidth]{data/PDF/naca_cl.pdf}
	\caption{\label{fig:cl_naca}}
	\end{subfigure}
	\caption{Time-periodic variation of (a)$C_D$ and (b)$C_L$ with respect to non-dimensional time $tU_\infty /c$. The results are compared to the ghost-cell IB method of \citet{mittalVersatileSharpInterface2008}.}
  \label{fig:naca_cdcl}
\end{figure}


==> sections/oscillating_t.tex <==
\subsection{Transversely oscillating cylinder in a quiescent fluid}
\label{sssec:oscillating_t}

A transversely oscillating cylinder within a quiscent background flow is tested. The domain of the flow is such that $Lx = Ly = 50D$ and the cylinder is placed at the center of the domain and is allowed to oscillate transversely such that the displacement of the cylinder is given by $\Delta x_c = 0.8D\sin(2\pi f_e t)$ where $f_e = 0.2$ is the oscilallting frequency. This gives us a Keulegan–Carpenter (KC) number of 5. The Keulegan-Carpenter number is described in \citet{dutschLowReynoldsnumberFlowOscillating1998} as $KC = 2\pi A/D$ where $A$ is the amplitude of oscillation and $D$ is the diameter of the cylinder. The above chosen values give us a maximum velocity of the cylinder such that $Re_D = 100$. The results are compared to that of \citet{dutschLowReynoldsnumberFlowOscillating1998}. For a moving (i.e. osscillating in this case) immersed solid the internal flow is significant as shown in figure \ref{fig:oscillating_domain_t} and is excluded while calculating the force at the interface through only considering points within the fluid phase. Figure \ref{fig:oscillating_streamlines_t} shows the streamlines of the velocity and results are similar to those captured by \citet{dutschLowReynoldsnumberFlowOscillating1998} at $KC = 5$ and $Re_D = 100$. The streamlines are shown at the point of maximum velocity of the cylinder, $U_{max} = KC f_e D$.

\begin{figure}\centering
        \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{images/oscillating_t_shedding.png}
        \caption{}
        \label{fig:oscillating_domain_t}
        \end{subfigure}
        \begin{subfigure}{0.45\linewidth}
        \includegraphics[width=\linewidth]{images/oscillating_t_streamlines.png}
        \caption{}
        \label{fig:oscillating_streamlines_t}
        \end{subfigure}
        \begin{subfigure}{0.9\linewidth}
        \includegraphics[width=\linewidth]{graphs/cylinder_oscillating_t/oscillate_t_cd.pdf}
        \caption{}
        \label{fig:oscillating_cd_t}
        \end{subfigure}
        \caption{This figure shows the (a) vortex shedding around an oscillating cylinder within a quiescent flow and (b) shows the velocity streamlines across the cylinder at the position of maximum velocity. Furthermore, (c) shows the coefficient of drag with respect to time.}
        \label{fig:oscillating_visit_t}
\end{figure}


Figure \ref{fig:oscillating_cd_t} shows the coefficient of drag. The simulation is run until statistically stationary and statistics are obtained after. Table \ref{tab:CD_cylinder_oscillating_t} shows the mean drag value of the oscillating cylinder within the quiescent fluid. Similar to other IBM formulations, the authors present a mean drag value that is an underprediction to the reference value by 102\%. This is again similar to what we have seen previously in the paper for other canonical cases in \S\ref{sec:filter_analysis} and \S\ref{sssec:freestream}. These results are well within the range of the reference values, and show an error that is minimal and similar or better to results shown by other IB formulations.

\begin{table}\centering
\begin{tabularx}{\linewidth}{bsbs}
\hline\hline
  	  			& $D/\Delta x$ & Filter kernel & $\overline{C}_{D}$       \\ \hline
 Present (T)   & 48           & Triangle       & -0.03  		              \\
 Present (T)   & 48           & Triweight      & -0.03  		              \\
 \citep{dutschLowReynoldsnumberFlowOscillating1998} & - & - & $2.15$  \\
\hline\hline
\end{tabularx}
\caption{This table shows the recorded $C_D$ for a cylinder transversely oscillating within a quiscent fluid recorded at 3 different resolutions and run using X filter kernel at $\delta f/2\Delta x = X$. The values are compared against the experimental studies of \citet{dutschLowReynoldsnumberFlowOscillating1998}.}
\label{tab:CD_cylinder_oscillating_t}
\end{table}


==> sections/uhlmann.tex <==
   Let us make the gross assumption that the volume fraction is \textbf{constant everywhere and is equal to one}. Although this is true a few filter widths away from the IB surface in the fluid side, this  assumption is \textbf{wrong} near the IB, \textbf{wrong} in the solid side, and breaks mass conservation. Nevertheless, let's assume that $\phi=1$ everywhere, and let's revisit steps (19) and (20):
\begin{enumerate}
  \item No-IB step:
    \begin{eqnarray}
      \frac{\overline{\mathbf{u}}^*-\overline{\mathbf{u}}^n}{\Delta t}=-\nabla\cdot(\overline{\mathbf{u}}\overline{\mathbf{u}})+\nu\nabla\cdot(\nabla\overline{\mathbf{u}})+\frac{1}{\rho_f}SGS
    \end{eqnarray}
  \item IB step
    \begin{eqnarray}
      \frac{\overline{\mathbf{u}}^\dagger-\overline{\mathbf{u}}^*}{\Delta t}&=&\frac{1}{\rho_f}\mathbf{f}^\dagger_{IB}\\
      &=&\sum_m S_{m} \delta(\mathbf{y}_m)\left\{\rho_f\frac{\mathbf{u}^{n+1}_{IB,m}-  \overline{\mathbf{u}}^*(\mathbf{y}_{m})}{\Delta t}\right\}g(\mathbf{x-y_m})
    \end{eqnarray}
\end{enumerate}
Aside from the additional SGS term, this is precisely Uhlmann's approach! Note that the SGS terms would also drop given sufficient resolution. We can make the following observations
\begin{itemize}
  \item Uhlmam's ``discretized dirac delta'', $\delta_h$, is in reality a filtering kernel $g$.
  \item The marker weight $\Delta V_l$ in Uhlamnn's work is ambiguous. In his 2005 paper, he doesn't give a satisfying answer for what it should be. He sets it to be equal to some local surface area multiplied by the mesh resolution $\Delta x$. In this derivation, we can clearly link this ``weight'' to the geometrical properties of the IB discretization:
    $$\Delta V_l= S_m \delta(\mathbf{y}_m)$$
    where $S_m$ is the surface area of a facet of the triangulation and $\delta(\mathbf{y}_m)$ is a length that can be computed from (30) and captures information about the local IB curvature.
  \item Ultimately, the lack of mass conservation (and appearance of seepage flow inside the solids) in Uhlamnn's method is due to an error in the estimation of the local fluid volume fraction.
\end{itemize}



